Compressive Sampling for Array Cameras

While design of high performance lenses and image sensors has long been the focus of camera development, the size, weight and power of image data processing components is currently the primary barrier to radical improvements in camera resolution. Here we show that Deep-Learning- Aided Compressive Sampling (DLACS) can reduce operating power on camera-head electronics by 20x. Traditional compressive sampling has to date been primarily applied in the physical sensor layer, we show here that with aid from deep learning algorithms, compressive sampling offers unique power management advantages in digital layer compression.

==> decomp_para_graph.tex <==
\paragraph{Decompression}
The eight-bit-integer array, $Comp_Q$, is the input of the decompression module, and is decompressed to be the decompressed raw-bayer data. In the decompression module, a pre-transpose  NN and a post-transpose NN are connected before and after the convolutional-2D-transpose layer.
The pre-transpose NN is a three-layer residual convolutional-2D NN, and its output, $dcomp_{\textrm{pre}}$, has the same dimension as $Comp_Q$. This NN can be conceptually viewed as compensating the loss due to the quantization process, and paves the way for the following steps of decompression. This NN is illustrated in Fig.~\ref{pd_NN}.
The convolutional-2D-transpose layer transforms $dcomp_{\textrm{pre}}$ into $dcomp$ which has the same dimension as the raw-bayer frame, $\textrm{Data}_{\textrm{in}}$.
The post-transpose NN is made of 20 convolutional-2D layers, 19 Batch-Normalization units and 10 Leaky-Relu activation units. Its output, $dcomp_{\textrm{pos}}$, has the same dimension as its input $dcomp$.  This NN can be viewed as carrying out post-processing to improve the quality of the output from the convolutional-2D-transpose layer, and its structure is illustrated in Fig.~\ref{pp_NN}.

\begin{figure*}[htb]
\includegraphics[width=0.9\textwidth]{res_block.pdf}
\caption{\label{pd_NN}(color online).  Pre-transpose NN structure: Conv $[k_x,\, k_y,\, n_c]$ represents the convolution-2D layer with a kernel of dimension $[k_x,\, k_y,\, n_c]$, stride equal to 1 and same padding, ReLU represents the rectified-linear-unit activation. The output of the third ReLU with $n_c = 1$ is broad-casted to the same $n_c$ of the input and added to the input, forming a residual NN block.}
\end{figure*}

\begin{figure*}[htb]
\includegraphics[width=0.9\textwidth]{post_process_NN_structure.pdf}
\caption{\label{pp_NN}(color online).  Post-transpose NN: Conv represents a convolution-2D layer, the convolutional kernel dimension is presented in square brackets as $[k_x,\, k_y,\, n_c]$, BN represents Batch normalization, Leaky ReLU represents the leaky-ReLU activation, Concat represents concatenating two tensors in the channel dimension, and Tanh represents the hyperbolic-tangent activation. The pre-stack module is presented in the top panel, and the stackable module is presented in the middle panel. The post-transpose NN made of the pre-stack module, eight stackable modules stacked together, and a few additional layers is presented in the bottom panel.}
\end{figure*}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk --shell-escape -pdf \"$_[0]\"" );
    }
}
